Strategies for Asymptotic Normalization

We present a technique to study normalizing strategies when termination is asymptotic, that is, it appears as a limit, as opposite to reaching a normal form in a finite number of steps. Asymptotic termination occurs in several settings, such as effectful, and in particular probabilistic computation -- where the limits are distributions over the possible outputs -- or infinitary lambda-calculi -- where the limits are infinitary normal forms such as Boehm trees. As a concrete application, we obtain a result which is of independent interest: a normalization theorem for Call-by-Value (and -- in a uniform way -- for Call-by-Name) probabilistic lambda-calculus.

==> 04_BT.tex <==
% !TEX root = main_2021.tex



%\newcommand{\opair}[2]{#1:#2}
%\newcommand{\pwred}{{\xredx{\pw}{}\ }}
\section{   More examples of Asymptotic Normalization}
\condinc{}{Depending on the context, non-termination of a program may be a problem, 
 or a desired property (witnessing the
liveness/progress of the  program). Infinitary computation and infinitary normal forms---in the form of  B{\"o}hm Trees for example---appear naturally also as a tool to study the behavior of programs  (\blue{observational and contextual equivalence}).
}



\subsection{ B{\"o}hm Trees  and Partial Normal Forms }\label{sec:BT}
We briefly  revisit  B{\"o}hm Trees, to show how their construction 
fits in our framework.

\paragraph{B{\"o}hm Trees.}
We adopt the definitions in \cite{AmadioCurien}(Sec. 2). The  B{\"o}hm Tree of a term $M$ is (the downward closure of) the set of the partial
normal forms of all reducts of $M$. 

\begin{Def}[Partial Normal Forms and B{\"o}hm Trees ]\label{def:BT}\hfill
	\begin{enumerate}
		\item 
		
		The set  $\PNF$ of \textbf{partial normal forms} is defined by
		\[\infer{\Omega\in \PNF}{} \quad \infer {\lam  x_1\dots x_n.xA_1\dots A_n\in
			\PNF}{A_1\in \PNF \dots A_p\in \PNF}
		\]
		
		$\PNF$ is a subset of partial $\lam$-terms, defined by $P:=\Omega\mid x\mid
		PP\mid \lam x.P$, and inherits its \textbf{order}, which is defined by	
		\[\infer{\Omega \leq P}{} \quad   \infer{P_1P_2\leq P'_1P'_2}{P_1\leq P'_1 &
			P_2\leq P'_2}
		\quad \infer{\lam x.P\leq \lam x.P'}{P\leq P'}\]
		
		$\PNF^\infty$ is the ideal completion of $\PNF$; its elements are called
		\textbf{B{\"o}hm Trees}.
		
		\item 
		The function  $\omega: \Lambda\red \PNF$  associates to each 
		term $M\in \Lambda$  its \emph{partial normal form} $\pnf M$ as follows:
		\[\pnf M = 
		\left\{
		\begin{array}{ll}
			\Omega& \mbox{ if } M\in \Hnf \\
			\lam \vec x. x \pnf {M_1}\dots \pnf {M_p}&\mbox{ if } M=\lam \vec x.
			xM_1...M_p
		\end{array}
		\right.\]
		\item \textbf{The B{\"o}hm Tree of }$M$ is defined as 
		\[\BT M := \bigcup\limits_{M\red^*N}  \downarrow \{\pnf N \}= \downarrow \{\pnf
		N \mid M\red^*N\}	\]
		where given a set $\mathcal S$, $\downarrow \mathcal S=\{ Q\in \PNF\mid Q\leq
		S\in \mathcal S \}$.
	\end{enumerate}
\end{Def}

\condinc{}{	\begin{Def}[B{\"o}hm Trees]\label{def:BT}
		
		The set  $\PNF$ of \textbf{partial normal forms} is defined by
		\[\infer{\Omega\in \PNF}{} \quad \infer {\lam  x_1\dots x_n.xA_1\dots A_n\in
			\PNF}{A_1\in \PNF \dots A_p\in \PNF}
		\]
		
		$\PNF$ is a subset of partial $\lam$-terms, defined by $P:=\Omega\mid x\mid
		PP\mid \lam x.P$, and inherits its \textbf{order}, which is defined by	
		\[\infer{\Omega \leq P}{} \quad   \infer{P_1P_2\leq P'_1P'_2}{P_1\leq P'_1 &
			P_2\leq P'_2}
		\quad \infer{\lam x.P\leq \lam x.P'}{P\leq P'}\]
		
		$\PNF^\infty$ is the ideal completion of $\PNF$; its elements are called
		\textbf{B{\"o}hm Trees}.
	\end{Def}
	
	\begin{Def}[Partial normal form of a term]
		Define $\omega: \Lambda\red \PNF$ which associate to each 
		term $M\in \Lambda$  its \emph{partial normal form} $\pnf M$ as follows:
		\[\pnf M = 
		\left\{
		\begin{array}{ll}
			\Omega& \mbox{ if } M\in \Hnf \\
			\lam \vec x. x \pnf {M_1}\dots \pnf {M_p}&\mbox{ if } M=\lam \vec x.
			xM_1...M_p
		\end{array}
		\right.\]
	\end{Def}
	
	
	\begin{Def}	[B{\"o}hm Trees] The B{\"o}hm Tree of $M$ is defined as 
		\[\BT M := \bigcup\limits_{M\red^*N}  \downarrow \{\pnf N \}= \downarrow \{\pnf
		N \mid M\red^*N\}	\]
		where given a set $\mathcal S$, $\downarrow \mathcal S=\{ Q\in \PNF\mid Q\leq
		S\in \mathcal S \}$.
	\end{Def}
}

%	\begin{Def}[B{\"o}hm Trees] The B{\"o}hm Tree of $M$ is defined as 
%		
%		
%		\[\BT M :=   \bigcup\limits_{M\red^*M'}  \{Q\in \PNF \mid Q\leq M'\} =
%\{Q\in \PNF\mid  Q\leq M', M\red^*M'\}  \]
%	\end{Def}
%	\begin{remark}	The above definition is equivalent (by Lemma \ref{lem:basics})
%to
%		\[\BT M := \bigcup\limits_{M\red^*N}  \downarrow \{\pnf N \}= \downarrow
%\{\pnf  N \mid M\red^*N\}	\]
%		where for a set $\mathcal S$ $\downarrow \mathcal S=\{ Q\in \PNF\mid Q\leq
%S\in \mathcal S \}$ is its downward closure.
%	\end{remark}



The following properties are standard to check
\begin{lemma}\label{lem:basics}Let $M,M'\in \Lambda$.
	\begin{itemize}
		
		\item[i] $M\red M'$ implies $\pnf M \leq \pnf{M'}$
		\item[ii] $\pnf M \leq M$
		\item[iii]  $Q\in \PNF$ and $ Q\leq M$ implies $Q\leq \pnf M$
	\end{itemize}
\end{lemma}

%	\begin{proof}By induction on the shape of $M$.
%	\end{proof}

\condinc{}{
	It holds  that 	
	\begin{theorem}\label{thm:BT}For each $M,N\in \Lambda$ 
		
		\begin{enumerate}
			\item[A.] If $M=_\beta N$ then $\BT M$ = $\BT N$
			\item[B.] If $\BT N = \BT M$ then $\BT{\cc \hole N} = \BT{\cc \hole M}$, for
			any context  $\cc$  which does not capture the free variables of neither $M$ nor
			$N$.
		\end{enumerate}		
	\end{theorem}
}

\paragraph{A QARS view.}
We   show that the  B{\"o}hm Tree of a term $M$  is the (unique) limit an asymptotically normalizing strategy, \ie the
limit of a \emph{single} reduction sequence.

Let us define $\obs: \Lambda\to \Nnf_\omega^\infty$ as \[\obs(M)= \downarrow
\{\pnf  {M}\} \]

By \Cref{lem:basics}, $\brack{(\Lambda, \redb),\obs }$	  is a QARS \footnote{In
	fact $\brack{(\Lambda, \redb),\omega }$ is an ARSI, in the sense of
	\cite{AriolaBlom02}}. 
%	We show that the  B{\"o}hm Tree of a term $M$ fits in our setting, and it can
%be defined as the limit a $\xredx{\pd}{\beta}$ reduction sequence.
%
The $\obs$-limit of a reduction sequence 
$\seq M$ is then
\[	   \sup_i\{\obs(M_i)\} = \bigcup_i  \downarrow \{\pnf  {M_i}\}	\]
It is immediate  that   $ \BT M$ is the l.u.b. of the set of limits $\wLim{(M,\redb)}$. We show that in fact $\BT M$ belongs to that set.
\paragraph{Asymptotic Completeness}
%\RED{\begin{prop}[$\los$-Factorization of $\redb$.]In $(\Lambda, \redb)$:\hfill
%	\begin{center}
%		$M \redb^*N$ implies $M \lsred^*\cdot \nlsred^* N$
%	\end{center}
%\end{prop}}

The reduction $\lsredb$ is  $\obs$-complete for $\redb$, by
\Cref{thm:ACompl},  because of 
$\los$-Factorization  of $\redb$ (\Cref{prop:out-factorization}) and $\neg\out$ neutrality.
\begin{lemma}[$\neg\out$ neutrality ]\label{prop:neutral_BT} If 
	$M\nlsred M'$ then  $\pnf {M} = \pnf {M'}$.
\end{lemma}

\begin{proof}By induction on $M$, observing that $M\in \Hnf$ iff  $M'\in \Hnf$,
	and that the two terms have the same shape.
\end{proof}



\begin{prop}[Asymptotic Completeness of $\lsred$]\label{prop:Oasymptotic_BT}
	$M \redb\conv{} \cpo{\r}$ implies 	$M \lsred\conv{} \cpo{\r}$
	
\end{prop}

\paragraph{Asymptotic Normalization.}
The reduction $\lsred$ is asymptotically complete, but not  normalizing. It has 
for example the diverging sequence $x(\Delta\Delta)(Iz) \lsred x(\Delta\Delta)(Iz) \lsred \dots$. We
proceed in a similar way as  in \Cref{sec:ANorm_CbV} (think  $\llRed$ vs $\llfull$).
We observe that $\xredx{\pd}{}$  is a deterministic reduction  which is
asymptotically complete for $ \lsred $. 

\condinc{}{
	\begin{lemma}
		Assume $M \lsred^nN $. Then  $M \xredx{\pd}{}^* N'$ and $N\lsred^*N'$, for some
		$N'$. Therefore $\pnf {N}\leq \pnf{N'}$
	\end{lemma}
}




\begin{lemma}\label{prop:POasymptotic_BT}
	$M \lsred\conv{} \cpo{\r}$ implies 	($M \xredx{\pd}{}\conv{} \cpo{\s}$ and
	$\cpo{\r} \leq \cpo{\s}$)
\end{lemma}
\begin{proof}
	The claim follows from the following fact, which is  easily proved by induction
	on $N$. Assume $M \lsred^*N $. Then  $M \xredx{\pd}{}^* N'$ and $N\lsred^*N'$,
	for some $N'$. Therefore $\pnf {N}\leq \pnf{N'}$, and so $ \cpo{\r} \leq
	\cpo{\s}$.
\end{proof}

By composing \Cref{prop:Oasymptotic_BT} and \ref{prop:POasymptotic_BT}  we
obtain (by  \refthm{complete})  
\begin{theorem}[Main]\label{} With the above definition of $\obs$, the   QARS
	$\brack{(\Lambda,\redb), \obs}$ satisfies, 
	for each $M \in \Lambda$:
	\begin{enumerate}
		\item[i] $\sem M$ is  defined 	
		\item[ii] $M \xredx{\pd}{}\conv{}  \sem {M}$
		
	\end{enumerate}
	Moreover   $\sem M =\BT{M}$.
\end{theorem}

\blue{\SLV
{
\subsection{$ \lam $-calculi with output}\label{sec:output_qars}
$ \lam $-calculi with output provides   an example 
---even though extremely simple---of asymptotic normalization in a calculus which has maximal limits, but not a greatest one.
% This allows us to give an example of  asymptotically normalizing strategy, which  produce a maximal element among the limits.
%The key  here  is divergence. 



 The calculus in \Cref{ex:output} can easily  be formalized
% by the system $(\alphabet\times \Lambda_{\print}, \wred)$
 as in \Cref{fig:}. %Terms $\Lambda_{\print}$ are as in \Cref{sec:lambda}.  
% We denote $\OutC \alphabet$ the $\lam$-calculus with output, where outputs are strings on the alphabet $\alphabet$.
 The grammar of terms is extended with a set of operators $\print{} \eq \{\print c , c\in \alphabet\}$. To each operator is associated the rule
   $\print c (P) \mapsto_{\print c} P$.
 
  The  elements of  the calculus are the pairs   $\m=(s:M)\in  \alphabet^* \times  \Lambda_{\print {}} $. 
   	For simplicity, we  only consider weak reduction,
which is lifted to pairs as follows.
%	\[\infer {(s:M)\wred (s.0:M')}{ M\wredx{\print 0}M'}   
%\quad  \infer {(s:M)\wred (s.1:M')}{ M\wredx{\print 1}M'}   
%\quad \infer {(s:M)\wred (s:M')}{M\wredbv M'}
%\]
\[\infer {(s:M)\wred (s.c:M')}{ M\wredx{\print c}M' & c\in \alphabet}   
\quad \infer {(s:M)\wred (s:M')}{M\wredbv M'}
\]
%{\small \[  (s: \ww\hole{ \print c (P)})  ~\wred ~  (c.s: \ww\hole{ P}) \quad    s:( \ww\hole {(\lam x.P)V})  \wred ~ ( s:\ww\hole{P\subs x V} )  \]}
We denote this calculus $\OutC \alphabet$.

The reduction is not confluent, %and moreover  the set of limits of a pair $\m$ may contain uncountably many different   elements. 
still,  the calculus  has interesting  regularity  properties. %, \RED{which appear when looking at the length of the strings.}


\paragraph{Observing convergence}
By fine tuning the notion of observation, one is able to establish the following, which is an instance of Weighted Random Descent.



%First, all maximal reduction sequences from the same pair $\m$ have the same number of steps. If the number of steps is finite, then all reduction sequences from $\m$ return the same value and  a string of the same length.
\begin{prop}[Converging computations]
	If  $\m$ has a terminating computation, \ie  $\m  \wred^*(s:V)$, then \emph{every} maximal sequence from $\m$  ends   in  a pair $(s':V)$ such that  $|s'| =|s|$. Moreover, all sequences  terminate    in  the same number of steps.	
\end{prop}
%\begin{proof}
%	If we assume $\alphabet $ to contain  a single character (just a tick to count the length) it is easy to see that 
%	$Out_{\alphabet}$ is $\obs$-diamond. The claim easily follows
%\end{proof}
%
Notice that if $\m$ has a  computation which diverges, all do. 


\paragraph{Observing possibly diverging computations}
Assume we  observe  the effect produced at any stage of   a partial (possibly diverging)
computation. Define 
\[\obs (s:M) \deff  s\]
Now the situation is more complex. %even if we only look at the lenght of the produced strings. 
\begin{example}
	Consider the term $M=(\Delta\Delta)(\dout{*}\dout{*})$, where $\dout{*}= \lam x.\print * (xx) $, and let
	$\m=(\epsilon:M)$. \begin{enumerate}
		\item By persistently choosing the   leftmost or rightmost  redex,  we would have, respectively,  $\wLim (\m,
		\lred)=\{\epsilon\} $ and  $\wLim (\m, \xredx{\rsym}{})=\{*^\omega\} $. 
		\item By choosing   a redex in 
		unspecified order, we have a countable number of $\wred$-sequences,
		leading to $\wLim (\m, \wred)=\{\epsilon,* , ** \dots\  *^\omega   \}     $
	\end{enumerate}
\end{example}
Fixing a deterministic evaluation order (point 1.) makes the limit easy to predict but rather arbitrary.
Let us  examine more closely 
 the  set  of limits associated with $\wred$. By moving to parallel reduction  $\xredx{\pw}{}$ (which is not difficult to define along the lines of  \Cref{fig:}) 
 we can establish that 
 the set of limits  $\xLim{\obs}{(M,\wred)}$ does have  maximal elements\footnote{The set $\{|\cpo s|\mid \cpo s\in \xLim{\obs_p}{(M,\wred)}\}\subseteq \Nat^\infty$ has a greatest element},
and indeed the multistep strategy  $\xredx{\pw}{}$  computes   one.



%All elements in $\wlim{M,\pwred}$  are maximal (because they all have the same length). 

\begin{prop}[Asymptotic Normalization]Consider the  QARS $\brack{\OutC \alphabet, \obs}$, defined  as above.  The reduction $\wred$ has a  (multistep)   $\obs$-normalizing   strategy.
	%because 
	% 	\begin{enumerate}
	% 	\item \emph{Asymptotic Completeness:}\\ $(s:M) \wred\conv{} \cpo{ n}$ implies 	\big($s:M \xredx{\pw}{}\ \conv{} \cpo {n'}$ and $|\cpo{s}| 	\leq |\cpo{s'}|$\big).
	% 	\item \emph{Unique Limit. } All elements in $\wlim{M,\pwred}$  are maximal (as they all have the same length)
	% \end{enumerate}
	
	%	\begin{itemize}
	%		\item  $\xredx{\pw}{}$ is $\obs_p$-complete for $\wred$. 
	%		\item All elements in $\wlim{M,\pwred}$  are maximal (as they all have the same length)
	%	\end{itemize}
\end{prop}
}{}}
%%%%%%%%%%%

\SLV{}{}{
\subsection{$ \lam $-calculi  with output}
Let us consider (weak) CbV $\lam$-calculus extended with an output operator. 

We first examine the issues which are related to  infinitary reduction looking at  a confluent  calculus, in which the output is  not a string, but simply an integer (think of it as a string on a single character). 


We then discuss the output $ \lam $-calculus of \Cref{ex:output}. This provides   an example 
---even though extremely simple---of asymptotic normalization in a calculus which has maximal limits, but not a greatest one.


\subsubsection{Payoff $\lam $-calculus.}\label{sec:payoff}
The  payoff $\lam $-calculus   (as in \cite{LagoG19}) extends the $\lam$-calculus with a 
	ticking operation. Its purpose is to  facilitate an  intensional analysis of programs, for instance by associating it to some  constructs in order to  perform cost analysis. 	
	

	
	The grammar of terms is extended  with a unary  operator $\tick$.
	We  represent
	the element in the calculus as pairs  ${n:M}$ of a counter $n\in \Nat$ and a term $M\in \Lambda_{\tick}$. Intuitively, 
	the term   $\tick   (P)$ increments the counter by $1$, and continues as $P$   \big(	${n:\tick(P)} \red {n+1:P}$\big).
%
	For simplicity, we  only consider weak reduction.
%	Let $\sredx{\tick}$ be the closure under  context $\ss\in
%	\{\ww,\leftc,\rightc\}$ of the rule $(\tick.P)\Root{\tick}P$
%	The reduction lifts to pairs as follows. 
%	\[\infer {(n:M)\sred (n+1:M')}{ M\sredx{\tick}M'}   
%	\quad \infer {(n:M)\sred (n:M')}{M\sredbv M'}
%	\]
%	
	Formally, let 
		 $\wredx{\tick}$ be  the closure under  context $\ww$ of the rule $(\tick.P)\Root{\tick}P$, and  let weak $\betav$ reduction $\wredbv$ be as usual.
	The reduction lifts to  $  (\Nat\times \Lambda_{\tick})  $  as follows 
	\[\infer {(n:M)\wred (n+1:M')}{ M\wredx{\tick}M'}   
	\quad \infer {(n:M)\wred (n:M')}{M\wredbv M'}
	\]
	Left and right reductions $\lred$ and  $\xredx{\rsym}{}$ %on $\Nat\times \Lambda_\tick $
	 can be  defined  similarly.
	
	\paragraph{Payoff of convergent computations.}
	Assume we observe (in $\Nat^\infty$) the payoff  associated to the computation of
	a value
	\[
	\left\{
	\begin{array}{ll}
		\obs_{v} (n:V) \deff n &  \\
		\obs_{v} (n:M) \deff 0 & \mbox{ if } M \not\in \Val 
	\end{array}
	\right.\]
	
	%\[\obs_{v} (n:V) =n  \quad\quad  \obs_{v} (n:M) =\bot  \mbox{ if } M \not\in
	%\Val \]
	%
It is easy to check that the  reduction $\wred$ satisfies the  $\obs_v$-diamond property.  Hence
	\begin{fact}Let $M \in \ \Lambda_{\tick}$. Assume 
 $M:0\wred^k (n:V)$, then \emph{every} maximal  $\wred$-reduction ends  after $k$
steps in the same pair $(n:V)$.
	\end{fact}
	
	
\paragraph{Payoff of diverging computations.}





	\begin{figure}
		\[\infer{\opair 0 M \pwred  \opair 0 {M'} }{M\Root{\betav} M'}  \quad \infer{\opair 0 M \pwred  \opair 1 {M'} }{M\Root{\tick}M'}
		\quad \infer   {\opair 0 V \pwred  \opair 0 {V} }{}\]
	\[	\infer{\opair 0 {P_1P_2}  \pwred    \opair {k_1+k_2} {P_1P_2}  }
		{  \opair 0 {P_1}  \pwred    \opair {k_1} {P_1} & \opair 0 {P_2}  \pwred    \opair {k_2} {P_2} } \quad
		\infer{ \opair {n} {M}  \pwred    \opair {n+k} {M'}}{n>0 & \opair 0 {M}  \pwred    \opair {k} {M'} }
		\]
		\caption{Parallel weak reduction on the payoff calculus}\label{fig:parallel_payoff}
	\end{figure}
%\begin{figure*}
%	\[\infer{\opair 0 M \pwred\ \opair 0 {M'} }{M\Root{\betav} M'}  \quad \infer{\opair 0 M \pwred\ \opair 1 {M'} }{M\Root{\tick}M'}
%	\quad \infer   {\opair 0 V \pwred\ \opair 0 {V} }{}\quad
%	\infer{\opair 0 {P_1P_2}  \pwred\   \opair {k_1+k_2} {P_1P_2}  }
%	{  \opair 0 {P_1}  \pwred\   \opair {k_1} {P_1} & \opair 0 {P_2}  \pwred\   \opair {k_2} {P_2} } \quad
%	\infer{ \opair {n} {M}  \pwred\   \opair {n+k} {M'}}{ \opair 0 {M}  \pwred\   \opair {k} {M'}}
%	\]
%	\caption{}
%\end{figure*}


Assume   that  we  observe  the payoff  also of partial (possibly diverging)
computations:
\[\obs_p (n:M) = n\]
Now the situation is more complex, and  $\wred$ has not a unique limit.
\begin{example}
	Consider the term $M=(\Delta\Delta)(\dtick\dtick)$, where $\dtick= \lam x.\tick(xx) $, and let
	$\m=(0:M)$. \begin{enumerate}
		\item By fixing  left or right  evaluation,  we have, respectively,  $\wLim (\m,
	\lred)=\{0\} $ and  $\wLim (\m, \xredx{\rsym}{})=\{\infty\} $. 
	\item By choosing   a redex in 
	 unspecified order, we have a countable number of $\wred$-sequences,
	leading to $\wLim (\m, \wred)=\{0,1, \dots\,\infty\} = \Nat^\infty $
	\end{enumerate}
\end{example}
%A possibility is to seek  an easy to predict  evaluation order, and  restrain $\tick$-reduction, by only allowing left or right reduction. 
Fixing a deterministic evaluation order (as in point 1.) makes the limit easy to predict but rather arbitrary.
Let us  examine more closely 
the  set  of limits associated with $\wred$. By moving to parallel reduction  $\xredx{\pw}{}$  (\Cref{fig:parallel_payoff})
we can establish that 
the set of limits  $\xLim{\obs}{(\m,\wred)}$ does have a greatest element---
  the multistep strategy  $\xredx{\pw}{}$  computes   it. Thus  $\sem {\m}$ is  the best possible payoff from $\m$.\\

%Instead of fixing a deterministic evaluation order, which is easy to predict but rather arbitrary, we can allow 
% non-deterministic choice of the weak
%redexes, and define $\sem {0:M}$ as the best possible payoff from $0:M$.
%Indeed,  a \emph{greatest} limit \emph{does exist} (as already clear from the example), and 
%parallel weak reduction $\xredx{\pw}{}$ computes such  a greatest limit.
% 

\condinc{}{
It is easily seen that  weak reduction $\xredx{\pw}{}$ is  $\obs$-complete  for
$\wred$ (point ii. below)


\renewcommand{\tr}{\mkern-6mu{}^*}
\begin{lemma}Let $n,n'\in \Nat$ and $\cpo {n}, \cpo{n'}\in \Nat^\infty$
\begin{enumerate}
	\item$0:M \wred^* {n:P}$ implies 	\big($0:M \xredx{\pw}{}^* {n':Q}$   and  ${n}
	\leq {n'}$\big) % $n:P \wred\tr {n:Q}$
	\item 	$k:M \wred\conv{} \cpo{ n}$ implies 	\big($k:M \xredx{\pw}{}\ \conv{} \cpo {n'}$ and $\cpo{n}
	\leq \cpo{n'}$\big)
\end{enumerate}
\end{lemma}

%Moreover, since   $\xredx{\pw}{}$ is deterministic, $\wlim{M,\pwred}$  contains  a unique limit, which by the previous lemma is the greatest element  $\sem M$ of 
% $\wlim{M,\wred}$ .
}

It is easy fo verify that  the conditions of \Cref{thm:ACompl} both hold:
	\begin{enumerate}
	\item[i] \emph{Asymptotic Completeness.}   
	  $(k:M) \wred\conv{} \cpo{ n}$ implies 	\big($k:M \xredx{\pw}{}\ \conv{} \cpo {n'}$ and $\cpo{n} 	\leq \cpo{n'}$\big).
	\item[ii] \emph{Unique Limit. } The reduction $ \xredx{\pw}{}  $ is deterministic.
\end{enumerate}

\condinc{}{Hence, for $\m=(0:M)$ and  $\sem {\m} $ 
\begin{itemize}
	\item $\sem {\m} $ is defined
	\item $\m \xredx{\pw}{}  \sem {\m} $
\end{itemize}
}
Hence  for each pair  $\m$ , 
$\sem {\m}$ 
is  defined, and $\m \xredx{\pw}{}  \conv{}  \sem {\m} $.
\begin{prop} 
	 Given the   QARS $\brack{(\Nat\times \Lambda_{\tick}, \wred), \obs_p}$,
%	 it is the  limit of the  $\xredx{\pw}{}$-sequence. 
	 %
 multistep reduction 
	$\xredx{\pw}{}$ is  asymptotically normalizing   for $\wred$.

\end{prop}




\subsubsection{ $\lam $-calculus with outputs} The calculus in   \Cref{ex:output} can be formalized in a similar way to the payoff calculus.
The  elements of  the calculus are the pairs   $\m=(s:M)\in  \alphabet^* \times  \Lambda_{\print {}} $. 
To each operator is associated the rule
$\print c (P) \mapsto_{\print c} P$.
Weak reduction,
which is lifted to pairs as follows.
%	\[\infer {(s:M)\wred (s.0:M')}{ M\wredx{\print 0}M'}   
%\quad  \infer {(s:M)\wred (s.1:M')}{ M\wredx{\print 1}M'}   
%\quad \infer {(s:M)\wred (s:M')}{M\wredbv M'}
%\]
\[\infer {(s:M)\wred (s.c:M')}{ M\wredx{\print c}M' & c\in \alphabet}   
\quad \infer {(s:M)\wred (s:M')}{M\wredbv M'}
\]
%{\small \[  (s: \ww\hole{ \print c (P)})  ~\wred ~  (c.s: \ww\hole{ P}) \quad    s:( \ww\hole {(\lam x.P)V})  \wred ~ ( s:\ww\hole{P\subs x V} )  \]}



%We consider again  two possible observations:
%
%\[ %\left\{
%\begin{array}{ll|}
%	\obs_{v} (s:V) \eq s &  \\
%	\obs_{v} (s:M) \eq \epsilon & \mbox{ if } M \not\in \Val 
%\end{array}
%%\right.
%\quad\quad
%	\obs_{p} (s:M) \eq s   \]

We define
\[\obs (s:M) \eq s\]
As already noted, $\wred$ is not confluent,  and given a pair $\m$,  the set of limits may contain uncountably many different   elements. Still,  the reduction  has interesting  regularity  properties, {which appear when looking at the length $|s|$ of the string in $s:M$.} Indeed,
 we can  transfer the  results from the payoff calculus.

%First, all maximal $\wred$-sequences have the same length.  Second, 
%maximal computations produce strings of the same length, in a  sense
%that is different in the case of convergence or  divergence.

%Let  $|s|$ be the length of the string $s$.


\paragraph*{Observing Convergence.} 
We can establish the following, which is an instance of Weighted Random Descent.



%First, all maximal reduction sequences from the same pair $\m$ have the same number of steps. If the number of steps is finite, then all reduction sequences from $\m$ return the same value and  a string of the same length.
\begin{prop}[Converging computations]
	If  $\m$ has a terminating computation, \ie  $\m  \wred^*(s:V)$, then \emph{every} maximal sequence from $\m$  ends   in  a pair $(s':V)$ such that  $|s'| =|s|$. Moreover, all sequences  terminate    in  the same number of steps.	
\end{prop}
%\begin{proof}
%	If we assume $\alphabet $ to contain  a single character (just a tick to count the length) it is easy to see that 
%	$Out_{\alphabet}$ is $\obs$-diamond. The claim easily follows
%\end{proof}
%




Notice that if $\m$ has a divergent computation, all reduction sequences from $\m$ diverge. %The  situation is similar  to that in \Cref{ex}. 
\paragraph*{Observing Divergence.}


Consider the set $\xLim{\obs_p}{(M,\wred)}$. Maximal elements exist, because the set $\{|\cpo s|\mid \cpo s\in \xLim{\obs_p}{(M,\wred)}\}$ has a greatest element.
The multistep reduction  $\xredx{\pw}{}$ (which is not difficult to define along the lines of that in \Cref{fig:parallel_payoff}) computes  a maximal limit, converging to a string of greatest length.


%All elements in $\wlim{M,\pwred}$  are maximal (because they all have the same length). 

%\begin{prop} Given the   QARS $\brack{(\alphabet^*\times \Lambda_{\{\print c\}}, \wred), \obs_p}$,  multistep reduction  %$\xredx{\pw}{}$ 
%	is   $\obs_p$ normalizing   for $\wred$.
	%because 
	% 	\begin{enumerate}
	% 	\item \emph{Asymptotic Completeness:}\\ $(s:M) \wred\conv{} \cpo{ n}$ implies 	\big($s:M \xredx{\pw}{}\ \conv{} \cpo {n'}$ and $|\cpo{s}| 	\leq |\cpo{s'}|$\big).
	% 	\item \emph{Unique Limit. } All elements in $\wlim{M,\pwred}$  are maximal (as they all have the same length)
	% \end{enumerate}
	
	%	\begin{itemize}
	%		\item  $\xredx{\pw}{}$ is $\obs_p$-complete for $\wred$. 
	%		\item All elements in $\wlim{M,\pwred}$  are maximal (as they all have the same length)
	%	\end{itemize}
%\end{prop}





\begin{prop}[Asymptotic Normalization] Given the  QARS $ \brack{(\alphabet^*\times \Lambda_{\print {}}, \wred), \obs}$
	 defined  as above, the  reduction $\xredx{\pw}{}$  is an asymptotic  (multi-step)  normalizing   strategy for 
	 $\wred$.
	%because 
	% 	\begin{enumerate}
	% 	\item \emph{Asymptotic Completeness:}\\ $(s:M) \wred\conv{} \cpo{ n}$ implies 	\big($s:M \xredx{\pw}{}\ \conv{} \cpo {n'}$ and $|\cpo{s}| 	\leq |\cpo{s'}|$\big).
	% 	\item \emph{Unique Limit. } All elements in $\wlim{M,\pwred}$  are maximal (as they all have the same length)
	% \end{enumerate}
	
	%	\begin{itemize}
	%		\item  $\xredx{\pw}{}$ is $\obs_p$-complete for $\wred$. 
	%		\item All elements in $\wlim{M,\pwred}$  are maximal (as they all have the same length)
	%	\end{itemize}
\end{prop}

}
%\RED{it is fairly easy to predict the order in
%	which expressions are evaluated so programs using sideeffecting IO can be fairly simple
%	to write and debug, if not to reason about formally
%	Both composites are evaluated in parallel or where there can be no interference between the two (which
%}


\newpage


==> 04_BT_short.tex <==
% !TEX root = main_2021.tex


\newcommand{\opair}[2]{\langle #1:#2 \rangle}
%\newcommand{\opair}[2]{#1:#2}
	\newcommand{\pwred}{{\xredx{\pw}{}\ }}
	
%\section{   More examples of Asymptotic Normalization}

\section{Asymptotic Normalization:  More Case Studies}
%\vspace*{-15pt}
We conclude by discussing the other examples of \Cref{sec:examples}. 
In this section we consider a CbV $\lam$-calculus extended with an output operator. For the sake of presentation, 
we take as output  not a string, but simply an integer (think of it as a string on a single character). While simple, this calculus allows us to illustrate the subtleties related to limits, and the use of our method.

In a similar way, one can revisit B{\"o}hm Trees as the limit of a specific asymptotic strategy---
we leave this to \Cref{sec:BT}.


\subsection{$\lambda$-calculus with output: the Payoff calculus} \label{sec:payoff}.


% 	\begin{itemize}
%	\item ${\ww\hole{\tick.P} \red_{\tick}  \ww\hole P} \\
%		 {\cc \hole{(\lambda x.M)V }\redbv \cc\hole{ M \subs x V} }\\
%	{\ww \hole{(\lambda x.M)V }\wredbv \ww\hole{ M \subs x V} }$\\
%		
%	
%	\item 	$ \red\,:=\, \redbv \cup \red_{\tick} $\quad
%	$ \wred\,:=\, \wredx{\betav} \cup \red_{\tick} $
%\end{itemize}

% 	\begin{itemize}
%	\item $\pair n {\ww\hole{\tick.P}} \red_{\tick}  \pair {n+1}{\ww\hole P} \\
%	\pair n {\cc \hole{(\lambda x.M)V }}\redbv \pair n  {\cc\hole{ M \subs x V} }\\
%	\pair n {\ww \hole{(\lambda x.M)V }}\wredbv \pair n {\ww\hole{ M \subs x V} }$\\
%	
%	
%	\item 	$ \red\,:=\, \redbv \cup \red_{\tick} $\quad
%	$ \wred\,:=\, \wredx{\betav} \cup \red_{\tick} $
%\end{itemize}

\begin{figure}
	\centering
	\begin{itemize}
	\item $\infer {\opair n {\ww\hole{\tick.P}} ~~\wredx{\tick} ~~  \opair {n+1}{\ww\hole P}}{} $\quad
	$ \infer {\opair n M \redbv \opair n{M'}}{M\redbv M'}
	\quad \infer {\opair n M\wredbv \opair n {M'})}{M\wredbv M'}
	$\\[4pt]
	
	\item 	$ \red\,:=\, \redbv \cup \wredx{\tick} $\quad
	$ \wred\,:=\, \wredx{\betav} \cup \red_{\tick} $
\end{itemize}
	\vspace*{-10pt} 	
\caption{Payoff reductions  ${\red},{\wred} ~\subseteq ~  (\Nat\times \Lambda_{\tick})  $ }\label{fig:payoff}

	{\small 	$\infer{\opair 0 M \pwred  \opair 0 {M'} }{M\Root{\betav} M'}  \quad \infer{\opair 0 M \pwred  \opair 1 {M'} }{M\Root{\tick}M'}
	\quad \infer   {\opair 0 V \pwred  \opair 0 {V} }{} \quad
	\infer{\opair 0 {P_1P_2}  \pwred    \opair {k_1+k_2} {P_1P_2}  }
	{  \opair 0 {P_1}  \pwred    \opair {k_1} {P_1} & \opair 0 {P_2}  \pwred    \opair {k_2} {P_2} } \quad
	\infer{ \opair {n} {M}  \pwred    \opair {n+k} {M'}}{n>0 & \opair 0 {M}  \pwred    \opair {k} {M'} }
	$}
\caption{Parallel weak reduction in the payoff calculus}\label{fig:parallel_payoff}
\end{figure}

\condinc{}{
\begin{itemize}
	\item $\pair n {\ww\hole{\tick.P}} \wredx{\tick}  \pair {n+1}{\ww\hole P} \\
	\pair n {\cc \hole{(\lambda x.M)V }}\redbv \pair n  {\cc\hole{ M \subs x V} }\\
	\pair n {\ww \hole{(\lambda x.M)V }}\wredbv \pair n {\ww\hole{ M \subs x V} }$\\
	
	
	\item 	$ \red\,:=\, \redbv \cup \wredx{\tick} $\quad
	$ \wred\,:=\, \wredx{\betav} \cup \red_{\tick} $
\end{itemize}
}





	
	

	The  payoff $\lam $-calculus   (called cost $\lam $-calculus in \cite{LagoG19} and \cite{GavazzoF21}) extends the $\lam$-calculus with a 
	ticking operation. Its purpose is to  facilitate an  intensional analysis of programs, for instance by associating it to some  constructs in order to  perform cost analysis. 	
	
	
	
	The set  of terms $\Lambda_{\tick}$ is extended  with a unary  operator $\tick$. 
	The element in the calculus as pairs  $\m = \opair n M$ of a counter $n\in \Nat$ and a term $M\in \Lambda_{\tick}$. Intuitively, 
	the term   $\tick   (P)$ increments the counter by $1$, and continues as $P$.
	Following \cite{GavazzoF21}, 
	effects only admit weak reduction. We let 
weak reduction 
$\wredx{\tick}$ to be   the closure under weak  context ($\ww$) of the rule $(\tick.P)\Root{\tick}P$ 
(left and right reductions $\lred$ and  $\xredx{\rsym}{}$ %on $\Nat\times \Lambda_\tick $
can be  defined  similarly.	)
	Letting     $\betav$ and  $\wredbv$ be as usual, 
	the reduction lifts to  $  (\Nat\times \Lambda_{\tick})  $  in the natural way, as  in \Cref{fig:payoff}. 
	
	Reduction 

	
	\SLV{}{
	\paragraph{Payoff of convergent computations.}
	Assume we observe (in $\Nat^\infty$) the payoff  associated to the computation of
	a value
	\[
	\left\{
	\begin{array}{ll}
		\obs_{v} (n:V) \deff n &  \\
		\obs_{v} (n:M) \deff 0 & \mbox{ if } M \not\in \Val 
	\end{array}
	\right.\]
	
	%\[\obs_{v} (n:V) =n  \quad\quad  \obs_{v} (n:M) =\bot  \mbox{ if } M \not\in
	%\Val \]
	%
	It is easy to check that the  reduction $\wred$ satisfies the  $\obs_v$-diamond property.  Hence
	\begin{fact}Let $M \in \ \Lambda_{\tick}$. Assume 
		$M:0\wred^k (n:V)$, then \emph{every} maximal  $\wred$-reduction ends  after $k$
		steps in the same pair $(n:V)$.
	\end{fact}
}
	
%	\paragraph{Payoff of diverging computations.}
	
	

	
	

	%\begin{figure*}
	%	\[\infer{\opair 0 M \pwred\ \opair 0 {M'} }{M\Root{\betav} M'}  \quad \infer{\opair 0 M \pwred\ \opair 1 {M'} }{M\Root{\tick}M'}
	%	\quad \infer   {\opair 0 V \pwred\ \opair 0 {V} }{}\quad
	%	\infer{\opair 0 {P_1P_2}  \pwred\   \opair {k_1+k_2} {P_1P_2}  }
	%	{  \opair 0 {P_1}  \pwred\   \opair {k_1} {P_1} & \opair 0 {P_2}  \pwred\   \opair {k_2} {P_2} } \quad
	%	\infer{ \opair {n} {M}  \pwred\   \opair {n+k} {M'}}{ \opair 0 {M}  \pwred\   \opair {k} {M'}}
	%	\]
	%	\caption{}
	%\end{figure*}
	

We  observe  the payoff  as follows:
\begin{center}
	$ 	\obs \opair  n M = n $
\end{center}
Weak reduction $\wred$ has not a unique limit. On the other side, 	the solution of fixing   a deterministic evaluation order (left or right, as in point 1. below) makes the limit easy to predict but rather arbitrary.
Let us see this with an example.
%$\wred$ has not a unique limit.
	\begin{example}
		Consider the term $M=(\Delta\Delta)(\dtick\dtick)$, where $\dtick= \lam x.\tick(xx) $, and let
		$\m=(0:M)$. \begin{enumerate}
			\item By fixing  left or right  evaluation,  we have, respectively,  $\wLim (\m,
			\lred)=\{0\} $ and  $\wLim (\m, \xredx{\rsym}{})=\{\infty\} $. 
			\item By choosing   a redex in 
			unspecified order, we have a countable number of $\wred$-sequences,
			leading to $\wLim (\m, \wred)=\{0,1, \dots\,\infty\} = \Nat^\infty $
		\end{enumerate}
	\end{example}
If we examine  more closely 
	the  set  of limits associated with $\wred$, we realize that $\xLim{\obs}{(\m,\wred)}$ does have a greatest element.
	Thus  $\sem {\m}$ can naturally be defined as   the best possible payoff from $\m$.
	By moving to parallel reduction  $\xredx{\pw}{}$  (\Cref{fig:parallel_payoff})
	we have a 
 multistep strategy  which   computes   it. 
	
	%Instead of fixing a deterministic evaluation order, which is easy to predict but rather arbitrary, we can allow 
	% non-deterministic choice of the weak
	%redexes, and define $\sem {0:M}$ as the best possible payoff from $0:M$.
	%Indeed,  a \emph{greatest} limit \emph{does exist} (as already clear from the example), and 
	%parallel weak reduction $\xredx{\pw}{}$ computes such  a greatest limit.
	% 
	
	\condinc{}{
		It is easily seen that  weak reduction $\xredx{\pw}{}$ is  $\obs$-complete  for
		$\wred$ (point ii. below)
		
		
		\renewcommand{\tr}{\mkern-6mu{}^*}
		\begin{lemma}Let $n,n'\in \Nat$ and $\cpo {n}, \cpo{n'}\in \Nat^\infty$
			\begin{enumerate}
				\item$0:M \wred^* {n:P}$ implies 	\big($0:M \xredx{\pw}{}^* {n':Q}$   and  ${n}
				\leq {n'}$\big) % $n:P \wred\tr {n:Q}$
				\item 	$k:M \wred\conv{} \cpo{ n}$ implies 	\big($k:M \xredx{\pw}{}\ \conv{} \cpo {n'}$ and $\cpo{n}
				\leq \cpo{n'}$\big)
			\end{enumerate}
		\end{lemma}
		
		%Moreover, since   $\xredx{\pw}{}$ is deterministic, $\wlim{M,\pwred}$  contains  a unique limit, which by the previous lemma is the greatest element  $\sem M$ of 
		% $\wlim{M,\wred}$ .
	}
	
	It is easy fo verify that  the conditions of \Cref{thm:ACompl} both hold:
	\begin{enumerate}
		\item[i] \emph{Asymptotic Completeness.}   
		$(k:M) \wred\conv{} \cpo{ n}$ implies 	\big($k:M \xredx{\pw}{}\ \conv{} \cpo {n'}$ and $\cpo{n} 	\leq \cpo{n'}$\big).
		\item[ii] \emph{Unique Limit. } The reduction $ \xredx{\pw}{}  $ is deterministic.
	\end{enumerate}
	
	\condinc{}{Hence, for $\m=(0:M)$ and  $\sem {\m} $ 
		\begin{itemize}
			\item $\sem {\m} $ is defined
			\item $\m \xredx{\pw}{}  \sem {\m} $
		\end{itemize}
	}
	Hence  for each pair  $\m$ , 
	$\sem {\m}$ 
	is  defined, and $\m \xredx{\pw}{}  \conv{}  \sem {\m} $.
	\begin{prop} 
		Given the   QARS $\brack{(\Nat\times \Lambda_{\tick}, \wred), \obs_p}$,
		%	 it is the  limit of the  $\xredx{\pw}{}$-sequence. 
		%
		multistep reduction 
		$\xredx{\pw}{}$ is  asymptotically normalizing   for $\wred$.
		
	\end{prop}
	
	
	
	
	\subsubsection{ $\lam $-calculus with outputs} The calculus in   \Cref{ex:output} can be formalized in a similar way to the payoff calculus.
	The  elements of  the calculus are the pairs   $\m=(s:M)\in  \alphabet^* \times  \Lambda_{\print {}} $. 
	To each operator is associated the rule
	$\print c (P) \mapsto_{\print c} P$.
	Weak reduction,
	which is lifted to pairs as follows.
	%	\[\infer {(s:M)\wred (s.0:M')}{ M\wredx{\print 0}M'}   
	%\quad  \infer {(s:M)\wred (s.1:M')}{ M\wredx{\print 1}M'}   
	%\quad \infer {(s:M)\wred (s:M')}{M\wredbv M'}
	%\]
	\[\infer {(s:M)\wred (s.c:M')}{ M\wredx{\print c}M' & c\in \alphabet}   
	\quad \infer {(s:M)\wred (s:M')}{M\wredbv M'}
	\]
	%{\small \[  (s: \ww\hole{ \print c (P)})  ~\wred ~  (c.s: \ww\hole{ P}) \quad    s:( \ww\hole {(\lam x.P)V})  \wred ~ ( s:\ww\hole{P\subs x V} )  \]}
	
	
	
	%We consider again  two possible observations:
	%
	%\[ %\left\{
	%\begin{array}{ll|}
	%	\obs_{v} (s:V) \eq s &  \\
	%	\obs_{v} (s:M) \eq \epsilon & \mbox{ if } M \not\in \Val 
	%\end{array}
	%%\right.
	%\quad\quad
	%	\obs_{p} (s:M) \eq s   \]
	
	We define
	\[\obs (s:M) \eq s\]
	As already noted, $\wred$ is not confluent,  and given a pair $\m$,  the set of limits may contain uncountably many different   elements. Still,  the reduction  has interesting  regularity  properties, {which appear when looking at the length $|s|$ of the string in $s:M$.} Indeed,
	we can  transfer the  results from the payoff calculus.
	
	%First, all maximal $\wred$-sequences have the same length.  Second, 
	%maximal computations produce strings of the same length, in a  sense
	%that is different in the case of convergence or  divergence.
	
	%Let  $|s|$ be the length of the string $s$.
	
	
	\paragraph*{Observing Convergence.} 
	We can establish the following, which is an instance of Weighted Random Descent.
	
	
	
	%First, all maximal reduction sequences from the same pair $\m$ have the same number of steps. If the number of steps is finite, then all reduction sequences from $\m$ return the same value and  a string of the same length.
	\begin{prop}[Converging computations]
		If  $\m$ has a terminating computation, \ie  $\m  \wred^*(s:V)$, then \emph{every} maximal sequence from $\m$  ends   in  a pair $(s':V)$ such that  $|s'| =|s|$. Moreover, all sequences  terminate    in  the same number of steps.	
	\end{prop}
	%\begin{proof}
	%	If we assume $\alphabet $ to contain  a single character (just a tick to count the length) it is easy to see that 
	%	$Out_{\alphabet}$ is $\obs$-diamond. The claim easily follows
	%\end{proof}
	%
	
	
	
	
	Notice that if $\m$ has a divergent computation, all reduction sequences from $\m$ diverge. %The  situation is similar  to that in \Cref{ex}. 
	\paragraph*{Observing Divergence.}
	
	
	Consider the set $\xLim{\obs_p}{(M,\wred)}$. Maximal elements exist, because the set $\{|\cpo s|\mid \cpo s\in \xLim{\obs_p}{(M,\wred)}\}$ has a greatest element.
	The multistep reduction  $\xredx{\pw}{}$ (which is not difficult to define along the lines of that in \Cref{fig:parallel_payoff}) computes  a maximal limit, converging to a string of greatest length.
	
	
	%All elements in $\wlim{M,\pwred}$  are maximal (because they all have the same length). 
	
	%\begin{prop} Given the   QARS $\brack{(\alphabet^*\times \Lambda_{\{\print c\}}, \wred), \obs_p}$,  multistep reduction  %$\xredx{\pw}{}$ 
	%	is   $\obs_p$ normalizing   for $\wred$.
	%because 
	% 	\begin{enumerate}
		% 	\item \emph{Asymptotic Completeness:}\\ $(s:M) \wred\conv{} \cpo{ n}$ implies 	\big($s:M \xredx{\pw}{}\ \conv{} \cpo {n'}$ and $|\cpo{s}| 	\leq |\cpo{s'}|$\big).
		% 	\item \emph{Unique Limit. } All elements in $\wlim{M,\pwred}$  are maximal (as they all have the same length)
		% \end{enumerate}
	
	%	\begin{itemize}
		%		\item  $\xredx{\pw}{}$ is $\obs_p$-complete for $\wred$. 
		%		\item All elements in $\wlim{M,\pwred}$  are maximal (as they all have the same length)
		%	\end{itemize}
	%\end{prop}
	
	
	
	

